Hybrid Pricing for Mobile Collaborative Internet Access

Mobile Collaborative Internet Access (MCA) enables mobile users to share their Internet through flexible tethering arrangements. This can potentially make better use of network resources. However, from a mobile network operator's (MNO's) viewpoint, it can either reduce revenue or increase congestion, and thus has been blocked by some MNOs in practice. We propose a hybrid pricing framework for MNOs who charge users separately for access and tethering. This scheme serves to coordinate the tethering decisions of mobile users with MNO network management objectives. We analyze the MNOs' equilibrium pricing strategies in both cooperative and competitive scenarios. In the cooperative scenario, at the equilibrium, each user's cost is independent of any chosen tethering links. We then characterize the optimal hybrid pricing strategies of MNOs in this scenario. For the competitive scenario, we formulate the MNOs' competitive interactions as a pricing game, and we show that MNO competition leads to equalized prices for users if an equilibrium exists but does not guarantee its existence. Both insights motivate a quantity competition game, which is shown to guarantee an equilibrium. Simulation results show that in scenarios of interest the proposed hybrid pricing schemes can double both MNOs' profit and users' payoff and such improvements increase with the degree of network heterogeneity.

==> Sec-illustrate.tex <==

\section{An Illustrative Example}\label{exa}



\com{updated 8:30}

To introduce the key model features and demonstrate some key insights, we consider an illustrative model with two MNOs $\{1,2\}$ and two MUs $\{1,2\}$. MNO 1 provides 4G LTE service to MU 1, and MNO 2 provides 3G service to MU 2. Each MNO announces a usage-based \textit{data price} and a usage-based \textit{tethering price} to its subscriber.
%
Two MUs are physically close by, so that they can share their Internet access (via tethering) through Wi-Fi Direct or Bluetooth.
The MUs cooperatively determine the direct downloaded data $\{x_i\}_{i\in\{1,2\}}$ and the received tethered data $\{y_i\}_{i\in\{1,2\}}$ ($y_i$ represents the amount of data MU $j(\neq i)$ downloads from the Internet and sends to MU $i$), in order to maximize their total payoff. Table \ref{para} shows the system parameters and the MUs' utility functions.

\rev{
\begin{table}[h]
\caption{MUs' Utility and System Parameters}
%\tiny
\centering
\begin{tabular}{c c c}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  MUs & MU 1& MU 2 \\
      \hline
      \hline
  Operational Cost (\$/MB)& 0.5 & 2.5 \\
\hline
  Capacity (MBps)& 8 & 3\\
\hline
  Utility (\$) & $5\cdot (x_1+y_1)^{0.3}$ & $10\cdot (x_2+y_2)^{0.3}$  \\
\hline
\end{tabular}
\label{para}
\end{table}}



We consider three pricing and tethering policies for MNOs:
\begin{itemize}
  \item \textbf{No-Tethering Pricing (NTP) Scheme}: The MNOs block the tethering service (equivalently,
setting the tethering price to be infinite). Hence, each MU can only download data from his own MNO. Each MNO optimizes its data price to maximize its profit.

  \item \textbf{Cooperative Data and Tethering Pricing Scheme}:
%  Each MNO prohibit tethering and sets an additional usage-based \textit{tethering price} for each MB her subscriber tethers to the other MU.
   Two MNOs cooperatively optimize  the data prices and tethering prices to maximize their total profit.

  \item \textbf{Competitive Data and Tethering Pricing Scheme}: Each MNO sets its own data price and
tethering price to maximize its own profit, taking into account the competition from the other MNO.
\end{itemize}



%
%Throughout these tethering policies, we can observe that properly designing the tethering policy can improve not only the MUs' total payoff but also the MNOs' profit.
 Tables \ref{res} shows the optimal (equilibrium) prices, data downloading amount (per time slot), and various performance metrics of the above three schemes.
 %For each tethering policy, we optimize the (equilibrium) pricing schemes (to be described). The resulting prices, data rates and performance are presented in Tables \ref{res}.

We have the following key observations:
\begin{itemize}
\item For both cooperative and competitive schemes, the optimal/equilibrium  tethering prices for two MUs are zero, and the data prices for two MUs are the same.
\item Both cooperative and competitive schemes achieve a higher MU payoff and a higher MNO profit than the NTP scheme.
\end{itemize}


%(i) For each scheme, the optimal/equilibrium  tethering prices for two MUs are zero and the data prices for two MUs are the same; (ii) both cooperative scheme and competitive scheme achieve a higher MUs' payoff and a higher MNOs' profit compared to the NTP scheme.

Next we will introduce the mathematical model in details, and provide derivations and discussion of the preceding observations.

